deepTerra -- AI Land Classification Made Easy

deepTerra is a comprehensive platform designed to facilitate the classification of land surface features using machine learning and satellite imagery. The platform includes modules for data collection, image augmentation, training, testing, and prediction, streamlining the entire workflow for image classification tasks. This paper presents a detailed overview of the capabilities of deepTerra, shows how it has been applied to various research areas, and discusses the future directions it might take.

==> discussion.tex <==
\section{Discussion} \label{disc}
\subsection{Implications of Findings}
\begin{itemize}
    \item Discuss the significance of the findings for garbage detection in satellite images and the broader field of environmental monitoring.
    \item Explore potential real-world applications of the most effective CNN architectures identified in the study.
\end{itemize}

\subsection{Comparison with Related Work}
\begin{itemize}
    \item Relate your findings to those from the literature review, highlighting consistencies and discrepancies.
    \item Discuss how your results contribute to the existing body of knowledge.
\end{itemize}

\subsection{Limitations}
\begin{itemize}
    \item Acknowledge any limitations of your study, such as dataset size, generalizability, or computational constraints.
    \item Suggest how these limitations could be addressed in future research.
\end{itemize}
